Enhancing Secret Key Generation in Block Fading Channels using Reconfigurable Intelligent Surfaces

Physical layer security (PLS) is superior to classical cryptography techniques due to its notion of perfect secrecy and independence to an eavesdropper's computational power. One form of PLS arises when Alice and Bob (the legitimate users) exchange signals to extract a common key from the random common channels. The drawback of extracting keys from wireless channels is the ample dependence on the dynamicity and fluctuations of the radio channel. However, some radio channels are constant such as line of sight (LoS) and can be estimated by Eve (an illegitimate user), or can be quite static in behaviour due to the presence low-mobility users thus restricting the amount of randomness. This in turn lowers the secret key rate (SKR) defined as the number of bits of key generated per channel use. In this work, we aim to address this challenge by using a reconfigurable intelligent surface (RIS) to produce random phases at certain carefully curated intervals such that it disrupts the channel in low entropy environments. We propose an RIS assisted key generation method, study its performance, and compare with benchmarks to observe the benefit of using an RIS while considering various important metrics such as key mismatch rate and average secret key throughput. Simulations are made to validate our theoretical findings showing an improvement in performance when an RIS is deployed.

==> extras.tex <==


\section{System Model}
\begin{figure}
    \centering
    \includegraphics[scale=0.44]{images/sysmodnew.png}
    \caption{System model with an access point Alice, receiver Bob, RIS Rose, and eavesdropper Eve.}
    \label{fig:sysmodel}
\end{figure}
%The common randomness between the two terminals (transmitter and receiver) that are exploited can be received signal strength (RSS), phases of channel, channel coefficients for channels with memory, second-scale statistics, etc. This work relies on two assumptions that have to be held randomness and reciprocity, otherwise this is a compromised set up and the keys produced at the transmitter and receiver even under perfect conditions of key extraction methods will either be predictable (not random) and/or mismatched. 


Consider a single antenna access point called Alice serving a single-antenna user called Bob while being assisted by an RIS called Rose equipped with $N$ elements. Rose is controlled by an RIS controller that communicates with Alice over a control link. There is also a passive eavesdropper called Eve trying to access the secret keys extracted by Alice and Bob from their common wireless channels, depicted in Fig. \ref{fig:sysmodel}. Eve knows the cryptosystem and the key establishing protocol, and aims to discover the key.
%\begin{figure}
 %   \centering
  %  \includegraphics[scale=0.4]{images/timedivide.png}
   % \caption{Time $\tau$ split into channel probing stage $\tau_C$  and secure transmission stage $\tau_T$.}
    %\label{fig:coherence}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/cascadedall.png}
    \caption{Time $\tau$ split into channel probing stage $\tau_C$  and secure transmission stage $\tau_T$}
    \label{fig:cascaded2}
    \label{fig:coherence}
\end{figure}

We assume a time-division duplexing (TDD) scheme, ensuring channel reciprocity. We assume block-fading channels in which all channels maintain constant values for $T$ symbols each symbols with duration $\tau_{sym}$ seconds and vary between blocks based on their respective distributions. Let $\tau_p=2\tau_{sym}$ represent the time required for one bidirectional  transmission between Alice and Bob. Both Alice and Bob transmit agreed-upon Gaussian pilot symbols in both directions to estimate their respective channels during a coherence interval of $T_S$ symbols, $T_S \leq T$.  The agreed upon pilot sequence from Alice to Bob 
$\mathbf{x} \in \mathbb{C}^{\frac{T_S}{2} \times 1}$  satisfy a power constraint given as  $\mathbb{E}[\|\mathbf{x}\|^{2}]\leq  P \tau_S$,  where $T_S=\frac{\tau_S}{\tau_{sym}}$ is the number of symbols in a single coherence period with unchanging RIS phase shift matrix.
In the even time slots, Alice sends pilot symbols and Bob and Eve receive 
\begin{align}
{y}_{i,t} =  (h_{ai} + \mathbf{h}_{ar}^H \boldsymbol{\Phi}_t \mathbf{h}_{ri} ) x_t + n_{i,t}, \quad i \in \{b, e\}
\end{align}  
 Bob sends pilot symbols ${x}_t \sim \mathcal{CN}(0,P)$ during odd time slots $t=1,3,5, \dots$ where Alice and Eve receive

\begin{align}
{y}_{i,t} =  (h_{bi} + \mathbf{h}_{br}^H \boldsymbol{\Phi}_t \mathbf{h}_{ri} ) x_t + n_{i,t}, \quad i \in \{a, e\}
\end{align}
 where ${h}_{ab}=h_{ba}$ is the Alice-Bob  direct scalar channel,
 $\mathbf{h}_{ir}  \in \mathbb{C}^{N\times 1}, i \in \{a,b\}$ is the channel from Alice $(a)$ or from Bob $(b)$ to Rose, 
 and $\mathbf{h}_{r,i} \sim \mathbb{C}^{N\times 1}, i \in \{a,b,e\}$ is the channel from Rose to all the other nodes (Alice, Bob, and Eve), $h_{ie},  i \in \{a,b\}$ is the direct channel between Alice and Bob to Eve, $\boldsymbol{\Phi}_t =\text{diag}([\alpha_{t,1} e^{j \theta_{t,1}}, \dots,$ $\alpha_{t,N}e^{j\theta_{t,N}}])\in \mathbb{C}^{N\times N}$ is the reflection matrix for Rose in time slot $t$, where $\alpha_{t,n}$ is the amplitude reflection coefficient which we assume to be equal to 1 motivated by advancements in lossless metasurfaces, and $\theta_{t,n}\in [0,2\pi]$ is the phase-shift applied by element $n$, %Here, $\text{diag}(\cdot)$ is an operator that transforms a vector of dimensions $d \times 1$ into a diagonal matrix of dimensions $d\times d$. We set $\alpha_{t,n}=1\ \forall n$, motivated by advancements in lossless metasurfaces. 
and the noise samples are distributed as  $n_{i,t}\sim \mathcal{CN}(0,\sigma_{ i}^2), i \in \{a,b,e\}$.

The independent Rayleigh {(block)} fading channels $h_{a,i}, \mathbf{h}_{ir}, \mathbf{h}_{ri}, i \in \{a,b,e\}$  can be written as
\begin{align}
\label{model_1}
&{h}_{ii}\sim \mathcal{CN}(0, \beta_{ii})\\
&\mathbf{h}_{ir}\sim \mathcal{CN}(0, \beta_{ir}\mathbf{I}_{N})\\
&\mathbf{h}_{ri}\sim \mathcal{CN}(0, \beta_{ri}\mathbf{I}_{N})
\end{align}
where  $\beta_{ii}, \beta_{ir},\beta_{ri} $ are the path loss factors.
In addition, the notion of block fading in this channel modelling indicates that these channels remain constant for a duration of one block (code length), and change independently between blocks.
 Next step is to process the received signals and estimate the overall channels in order to gain correlated observations at Alice and Bob and extract the key.

\subsection{Channel Estimation}


%The key exchange protocol happen at the same time as pilot transmission, learning channel parameters from both ends.
%Making sure the channels are learnt properly because of reciprocity.

Let the estimates of the combined channels at each node (Alice, Bob, or Eve) be defined  as
\begin{align}
    \hat{h}_{a,t}&=h_{a,t}+ \frac{n_{a,t}}{x_t}=(h_{ba} + \mathbf{h}_{br}^H \boldsymbol{\Phi}_t \mathbf{h}_{ra} ) + \frac{n_{a,t}}{x_t}.\\
        \hat{h}_{b,t}&={h}_{b,t}+ \frac{n_{b,t}}{x_t}=(h_{ab} + \mathbf{h}_{ar}^H \boldsymbol{\Phi}_t \mathbf{h}_{rb} ) + \frac{n_{b,t}}{x_t}.\\
     \hat{h}_{e,t}&={h}_{e,t}+\frac{n_{e,t}}{x_t}=(h_{be} + \mathbf{h}_{br}^H \boldsymbol{\Phi}_t \mathbf{h}_{re} ) + \frac{n_{e,t}}{x_t}.\\
      \hat{h}_{e,t+1}&={h}_{e,t+1}+ + \frac{n_{e,t+1}}{x_{t+1}}=(h_{ae} + \mathbf{h}_{ar}^H \boldsymbol{\Phi}_{t+1} \mathbf{h}_{re} ) + \frac{n_{e,t+1}}{x_{t+1}}.
\end{align}
Note that $\hat{h}_{i,t} \sim \mathcal{CN}(0, \hat{\sigma}_i^2), i \in \{a,b,e\}$. Moreover, $\boldsymbol{\Phi}_{t}=\boldsymbol{\Phi}_{t+1}$ for $t$ odd.
In case, $T_s$ ping-pong transmissions occurred in which the channel was not disrupted by Rose or the switching rate is slow, i.e. $h_{a,t}=h_a, t=1,\dots, T_s$, then we can have an average of channel estimates as 
\begin{align}
\bar{h}_{a}=h_{a} +\frac{\sum_{t=1}^{T_s} n_{a,t}/x_{t}}{T_s}
\end{align}


 \subsection{Secrecy Rate Analysis}

To have a guarantee for secret transmission, we utilize the lower-bound of the secret key rate to defined as 

\begin{align}
 R_{K}^{LB}=  I(h_{A}; h_{B})-\text{min}[I(h_{A};h_{E,A}),I(h_{B};h_{E, B})]  \leq R_{K}.
 \end{align}
 A closed form expression can be given as \cite{lowerboundKey} in the Lemma.
 \begin{lemma} Given equal estimation error variances  at Alice, Bob, and Eve i.e. $\hat{\sigma}_a^2=\hat{\sigma_B}^2=\hat{\sigma}_E^2=\sigma^2$, the lowerbound for the secret key rate under an RIS assisted system simplifies to
 \begin{align}
R_{K}^{LB}=\frac{1}{\tau_S}\log_2\bigg(\frac{\rho^2_{a,b}-\rho_{a,b}(\rho_{a,e}+\rho_{b,e})}{(\rho_{a,e}+\rho_{b,e}+\sigma^2)(2\rho_{a,b}+\sigma^2)}\bigg),
 \end{align}

 \end{lemma}
 \begin{IEEEproof}
 The proof can be found in \cite{lowerboundKey}.
 \end{IEEEproof}

 
 %Alice and Bob can
%generate a key with rate
%\begin{align}
%R_K= \frac{\tau_{sym}}{\tau}I(\hat{h}_{A};\hat{h}_{B})
%\end{align}  

Let us define the following correlation function as $\rho_{i,j}=\mathbb{E}\{h_ih_j^*\}$, $i\in\{a,b\},j\in\{b,e\}$ where the expectation is taken over random channels and phases. We can obtain the following theorem
\begin{theorem}
For the correlations between Alice and Bob $\rho_{a,b}$, Alice and Eve $  \rho_{a,e}$, and Bob and Eve $\rho_{b,e}$, we have the closed-form expressions as 
    \begin{align}
     \rho_{a,b}&=\mathbb{E}\{h_ah_b^*\}=\beta_{ab}+N\beta_{ar}\beta_{br}
    \\
             \rho_{a,e}&=\mathbb{E}\{h_Ah_E^*\}=\beta_{ae}+N\beta_{ar}\beta_{re}
    \\ 
      \rho_{b,e}&=\mathbb{E}\{h_B h_E^*\}=\beta_{be}+N\beta_{br}\beta_{re}
 \end{align}
  
\end{theorem}
\begin{IEEEproof}
    Using the same argument in \cite{impactofPhaseRandomIRS}, we have that when $N$ is large and the IRS configuration is random, that the expression $g_{ab}=\sum_n \phi_{t,n} h_{ar,n}h_{rb,n}$ follows a complex normal distribution with mean zero and variance $N\beta_{ar}\beta_{br}$
\end{IEEEproof}

==> images/covariance.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=3.115in,
height=2.221in,
at={(0.529in,0.445in)},
scale only axis,
xmin=0,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={N},
ymin=0,
ymax=200,
ylabel style={font=\color{white!15!black}},
ylabel={Covariance},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={at={(0.166,0.731)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
1	1.99691739133418\\
2	3.56548582527998\\
3	5.15444835848407\\
4	6.39657694626165\\
5	8.8576447186024\\
6	10.9744133197522\\
7	11.7683813878451\\
8	12.4281214129949\\
9	15.4621277194629\\
10	15.6683410460326\\
11	18.1196342440871\\
12	20.2605701485819\\
13	22.9465137595657\\
14	23.8536856752298\\
15	24.873825233413\\
16	27.7220181507829\\
17	28.4221565487783\\
18	30.2898359290454\\
19	32.4012254730751\\
20	33.8194151672351\\
21	34.5808899896443\\
22	36.0271479597387\\
23	38.8870241258664\\
24	39.0817281716718\\
25	41.6562136419595\\
26	43.0731822582097\\
27	48.1989607201924\\
28	46.6925109615662\\
29	45.3843087131587\\
30	52.0972339836801\\
31	51.1238001452465\\
32	51.1154493971701\\
33	57.5147203254183\\
34	57.1654658315044\\
35	59.0195304340707\\
36	57.5834204874407\\
37	60.4059853779117\\
38	61.6555656688401\\
39	63.9104887892594\\
40	64.2654771456634\\
};
\addlegendentry{Monte Carlo}

\addplot [color=red, dashdotted, line width=2.0pt]
  table[row sep=crcr]{%
1	2\\
2	3.5\\
3	5.125\\
4	6.78125\\
5	8.4453125\\
6	10.111328125\\
7	11.77783203125\\
8	13.4444580078125\\
9	15.1111145019531\\
10	16.7777786254883\\
11	18.4444446563721\\
12	20.111111164093\\
13	21.7777777910233\\
14	23.4444444477558\\
15	25.1111111119389\\
16	26.7777777779847\\
17	28.4444444444962\\
18	30.111111111124\\
19	31.777777777781\\
20	33.4444444444452\\
21	35.1111111111113\\
22	36.7777777777778\\
23	38.4444444444445\\
24	40.1111111111111\\
25	41.7777777777778\\
26	43.4444444444444\\
27	45.1111111111111\\
28	46.7777777777778\\
29	48.4444444444444\\
30	50.1111111111111\\
31	51.7777777777778\\
32	53.4444444444444\\
33	55.1111111111111\\
34	56.7777777777778\\
35	58.4444444444444\\
36	60.1111111111111\\
37	61.7777777777778\\
38	63.4444444444444\\
39	65.1111111111111\\
40	66.7777777777778\\
};
\addlegendentry{Theoretic}

\addplot [color=black, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	1.97141628660773\\
2	3.35736009422341\\
3	5.12036708115483\\
4	6.86656148023156\\
5	8.16773837866379\\
6	10.0796417250342\\
7	11.656640566368\\
8	13.2848295268205\\
9	14.8610806275519\\
10	16.8005966845527\\
11	18.5155691602355\\
12	19.8434709161084\\
13	21.1420412466064\\
14	23.0719058390783\\
15	25.3531943084376\\
16	26.5608258964406\\
17	28.1405162517242\\
18	31.0712337803681\\
19	31.9348051915515\\
20	33.0372184717386\\
21	34.896602003278\\
22	36.699360994326\\
23	38.5276196988368\\
24	40.0036451072458\\
25	41.3567942486287\\
26	42.4822323750538\\
27	46.1826773813329\\
28	46.8735434613689\\
29	49.002128544789\\
30	50.034689993657\\
31	51.3012416098193\\
32	53.0478260897597\\
33	56.2248766832148\\
34	57.4535678215025\\
35	57.6715555677745\\
36	60.2417286769359\\
37	63.7337164575708\\
38	63.1325983132487\\
39	64.9266981648239\\
40	66.487539291438\\
41	69.5833393273239\\
42	69.1480164942352\\
43	73.4995532772452\\
44	72.9821581967847\\
45	74.395937213545\\
46	76.1695942361982\\
47	78.6282168198801\\
48	78.2642228060845\\
49	82.6125713574727\\
50	83.4943997320716\\
51	86.8251444827763\\
52	86.6917608682057\\
53	86.8862973816644\\
54	91.5520713798421\\
55	91.0105737500231\\
56	94.1258569416185\\
57	97.3879304788887\\
58	98.2624345364414\\
59	97.6732411324952\\
60	97.0375485510811\\
61	98.9913022979557\\
62	104.423052334726\\
63	104.707443536256\\
64	105.996550318195\\
65	106.514045533208\\
66	112.92980283944\\
67	112.31373099305\\
68	114.735576249011\\
69	115.832396232344\\
70	119.765330850425\\
71	118.492525440214\\
72	120.65843404411\\
73	125.509053141792\\
74	122.41842892586\\
75	126.138777187334\\
76	128.602658380505\\
77	128.261974617919\\
78	127.060667634632\\
79	134.10825089219\\
80	131.622413524118\\
81	138.624709229947\\
82	137.826262514978\\
83	141.35776428465\\
84	137.540765752772\\
85	141.815137107223\\
86	141.65077694791\\
87	146.584921532585\\
88	147.31348740005\\
89	147.836613375888\\
90	151.065479645582\\
91	155.128875419267\\
92	150.321922777159\\
93	153.404691486852\\
94	156.759929982065\\
95	158.578637298276\\
96	162.264031370368\\
97	164.222166056187\\
98	159.378001003957\\
99	163.893039253158\\
100	163.156264708771\\
};
\addplot [color=red, dashdotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	2\\
2	3.5\\
3	5.125\\
4	6.78125\\
5	8.4453125\\
6	10.111328125\\
7	11.77783203125\\
8	13.4444580078125\\
9	15.1111145019531\\
10	16.7777786254883\\
11	18.4444446563721\\
12	20.111111164093\\
13	21.7777777910233\\
14	23.4444444477558\\
15	25.1111111119389\\
16	26.7777777779847\\
17	28.4444444444962\\
18	30.111111111124\\
19	31.777777777781\\
20	33.4444444444452\\
21	35.1111111111113\\
22	36.7777777777778\\
23	38.4444444444445\\
24	40.1111111111111\\
25	41.7777777777778\\
26	43.4444444444444\\
27	45.1111111111111\\
28	46.7777777777778\\
29	48.4444444444444\\
30	50.1111111111111\\
31	51.7777777777778\\
32	53.4444444444444\\
33	55.1111111111111\\
34	56.7777777777778\\
35	58.4444444444444\\
36	60.1111111111111\\
37	61.7777777777778\\
38	63.4444444444444\\
39	65.1111111111111\\
40	66.7777777777778\\
41	68.4444444444444\\
42	70.1111111111111\\
43	71.7777777777778\\
44	73.4444444444445\\
45	75.1111111111111\\
46	76.7777777777778\\
47	78.4444444444445\\
48	80.1111111111111\\
49	81.7777777777778\\
50	83.4444444444444\\
51	85.1111111111111\\
52	86.7777777777778\\
53	88.4444444444445\\
54	90.1111111111111\\
55	91.7777777777778\\
56	93.4444444444444\\
57	95.1111111111111\\
58	96.7777777777778\\
59	98.4444444444445\\
60	100.111111111111\\
61	101.777777777778\\
62	103.444444444444\\
63	105.111111111111\\
64	106.777777777778\\
65	108.444444444444\\
66	110.111111111111\\
67	111.777777777778\\
68	113.444444444444\\
69	115.111111111111\\
70	116.777777777778\\
71	118.444444444444\\
72	120.111111111111\\
73	121.777777777778\\
74	123.444444444444\\
75	125.111111111111\\
76	126.777777777778\\
77	128.444444444444\\
78	130.111111111111\\
79	131.777777777778\\
80	133.444444444444\\
81	135.111111111111\\
82	136.777777777778\\
83	138.444444444444\\
84	140.111111111111\\
85	141.777777777778\\
86	143.444444444444\\
87	145.111111111111\\
88	146.777777777778\\
89	148.444444444444\\
90	150.111111111111\\
91	151.777777777778\\
92	153.444444444444\\
93	155.111111111111\\
94	156.777777777778\\
95	158.444444444444\\
96	160.111111111111\\
97	161.777777777778\\
98	163.444444444444\\
99	165.111111111111\\
100	166.777777777778\\
};
\end{axis}

\begin{axis}[%
width=4.027in,
height=2.881in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
